Dense RGB SLAM with Neural Implicit Maps

There is an emerging trend of using neural implicit functions for map representation in Simultaneous Localization and Mapping (SLAM). Some pioneer works have achieved encouraging results on RGB-D SLAM. In this paper, we present a dense RGB SLAM method with neural implicit map representation. To reach this challenging goal without depth input, we introduce a hierarchical feature volume to facilitate the implicit map decoder. This design effectively fuses shape cues across different scales to facilitate map reconstruction. Our method simultaneously solves the camera motion and the neural implicit map by matching the rendered and input video frames. To facilitate optimization, we further propose a photometric warping loss in the spirit of multi-view stereo to better constrain the camera pose and scene geometry. We evaluate our method on commonly used benchmarks and compare it with modern RGB and RGB-D SLAM systems. Our method achieves favorable results than previous methods and even surpasses some recent RGB-D SLAM methods.The code is at poptree.github.io/DIM-SLAM/.

==> figure/tum.tex <==
\begin{figure}[t]
\begin{center}

\begin{subfigure}{0.48\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0.0cm 0cm 0cm}, clip]{figure/tum/tum-fr1-desk.png}
  \caption*{\texttt{fr1/desk}}
\end{subfigure}
\begin{subfigure}{0.48\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/tum/tum-xyz-vis.png}
  \caption*{\textit{fr2/xyz}}
\end{subfigure}



\end{center}
\vspace{-3mm}
 \caption{The visualization of scenes on \textit{TUM RGB-D} dataset.}
 % \ping{make the letter `Ours', `iMAP' larger..}
\label{fig:tum_vis}
\vspace{-4mm}
\end{figure}




==> table/replica_small.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table}[t]
\small
\begin{center}
\begin{tabular}{clccccccccc}
\toprule


& & \texttt{o-0}& \texttt{o-1}& \texttt{o-2} & \texttt{o-3}& \texttt{o-4} & \texttt{r-0} & \texttt{r-1} & \texttt{r-2} & Avg.\\
\midrule
NICE-SLAM & \multirow{4}{*}{ATE RMSE[cm]$\downarrow$} & 1.02 & 3.91 &  1.76 & 6.10 & 11.9 & 4.37 & 2.76 & 3.54 & 4.4\\
DROID-SLAM & & \textbf{0.25} & 0.45          & \textbf{0.32} & 0.44          & 0.37          & \textbf{0.35} & \textbf{0.33} & \textbf{0.28} & \textbf{0.35}\\
Ours(Small) &         & 0.89        & 0.72 & 1.11          & 0.75 & 0.92 & 0.84 & 1.22 & 0.66  & 0.89\\
Ours(Default) &         & 0.67        & \textbf{0.37} & 0.36          & \textbf{0.33} & \textbf{0.36} & 0.48 & 0.78 & 0.35 & 0.46\\
\midrule \midrule
\multirow{3}{*}{iMAP} & \textbf{Acc.}[cm]$\downarrow$ &5.87&3.71&4.81&4.27&4.83&3.58&3.69&4.68&4.43\\
                      & \textbf{Comp.}[cm]$\downarrow$& 6.11 & 5.26& 5.65& 5.45&6.59& 5.06&4.87&5.51 &5.56\\
                      & \textbf{Comp. Ratio}[$\leq5$cm$\%$]$\uparrow$&77.71&79.64&77.22&77.34&77.63&83.91&83.45&75.53&79.06\\
\\ %\midrule
\multirow{3}{*}{NICE-SLAM} & \textbf{Acc.}[cm]$\downarrow$&\textbf{2.26}&2.50&3.82&3.50&2.77&2.73&\textbf{2.58}&\textbf{2.65}&\textbf{2.85}\\
                      & \textbf{Comp.}[cm]$\downarrow$ & \textbf{2.02} & 2.36 & \textbf{3.57} & \textbf{3.83} & \textbf{3.84} & \textbf{2.87} &\textbf{2.47} &\textbf{3.00} & \textbf{3.00}\\
                      & \textbf{Comp. Ratio}[$\leq5$cm$\%$]$\uparrow$&\textbf{94.93}&\textbf{92.61}&\textbf{85.20}&\textbf{82.98}&\textbf{86.14}&\textbf{90.93}&\textbf{92.80}&\textbf{89.07}&\textbf{89.33}\\
\\ %\midrule
\multirow{3}{*}{DI-Fuison} & \textbf{Acc.}[cm]$\downarrow$&70.56&\textbf{1.42}&\textbf{2.11}&\textbf{2.11}&\textbf{2.02}&\textbf{1.79}&49.00&26.17&19.40\\
                      & \textbf{Comp.}[cm]$\downarrow$&3.58&\textbf{2.20}&4.83&4.71&5.84&3.57&39.40&17.35&10.19\\
                      & \textbf{Comp. Ratio}[$\leq5$cm$\%$]$\uparrow$&87.17&91.85&80.13&79.94&80.21&87.77&32.01&45.61&72.96\\
\midrule
\multirow{3}{*}{DROID-SLAM} & \textbf{Acc.}[cm]$\downarrow$&3.26&2.92&4.90&\textbf{4.47}&5.35&4.01&4.53&\textbf{4.40}&4.23\\
                      & \textbf{Comp.}[cm]$\downarrow$&4.22&5.54&7.97&7.77&6.80&7.10&5.72&9.43&6.82\\
                      & \textbf{Comp. Ratio}[$\leq5$cm$\%$]$\uparrow$&77.57&72.95&59.85&62.30&66.50&68.35&71.68&68.76&68.50\\
\\
\multirow{3}{*}{Ours(Small)} & \textbf{Acc.}[cm]$\downarrow$&2.81&2.33&5.02&5.61&4.83&\textbf{3.61}&4.12&6.06&4.29\\
& \textbf{Comp.}[cm]$\downarrow$&2.71&3.25&6.63&6.33&6.11&5.97&5.31&7.43&5.46\\
& \textbf{Comp. Ratio}[$\leq5$cm$\%$]$\uparrow$&88.56&84.7&71.40&72.54&73.23&81.12&76.94&70.85&77.41\\
\\
\multirow{3}{*}{Ours(Default)} & \textbf{Acc.}[cm]$\downarrow$&\textbf{2.60}&\textbf{2.02}&\textbf{4.50}&5.43&\textbf{4.57}&3.68&\textbf{3.64}&5.84&\textbf{4.03}\\
                      & \textbf{Comp.}[cm]$\downarrow$&\textbf{2.65}&\textbf{3.31}&\textbf{6.09}&\textbf{5.98}&\textbf{5.81}&\textbf{5.32}&\textbf{4.72}&\textbf{5.70}&\textbf{4.20}\\
                      & \textbf{Comp. Ratio}[$\leq5$cm$\%$]$\uparrow$&\textbf{89.57}&\textbf{84.9}&\textbf{75.3}&\textbf{73.48}&\textbf{76.62}&\textbf{82.2}&\textbf{80.4}&\textbf{74.44}&\textbf{79.6}\\

\bottomrule

\end{tabular}
\caption{Quantitative results on the \textit{Replica} dataset. Here, `o-x' and `r-x' denote \texttt{office-x} and \texttt{room-x} sequence respectively. The top part shows the results of tracking, and the lower part shows the results of mapping. DROID-SLAM and our method work with the RGB inputs, while the others are all based on RGB-D data. The best results in RGB and RGB-D SLAMs are \textbf{bolded} respectively.}
\vspace{-2mm}
\label{table:replicasmall}
\vspace{-4mm}
\end{center}
\end{table}

==> table/tumandscannet.tex <==
\begin{table}[t]
\caption{Camera Tracking Results on TUM-RGBD.}
\label{table:replica}
\begin{center}
\begin{tabular}{llll}
\multicolumn{1}{c}{method} & \multicolumn{1}{c}{\texttt{scene0207}} & \multicolumn{1}{c}{\texttt{fr2/xyz}} & \multicolumn{1}{c}{\texttt{fr3/office}}  \\
\hline \\
 iMAP* &7.2 &2.1 &9.0\\
 NICE-SLAM &2.7 &1.8 &3.0  \\
 Droid-slam &- & -&- \\
 Ours & &- & - \\

\end{tabular}
\end{center}
\end{table}
